Crowdsourcing in Computer Vision

Computer vision systems require large amounts of manually annotated data to properly learn challenging visual concepts. Crowdsourcing platforms offer an inexpensive method to capture human knowledge and understanding, for a vast number of visual perception tasks. In this survey, we describe the types of annotations computer vision researchers have collected using crowdsourcing, and how they have ensured that this data is of high quality while annotation effort is minimized. We begin by discussing data collection on both classic (e.g., object recognition) and recent (e.g., visual story-telling) vision tasks. We then summarize key design decisions for creating effective data collection interfaces and workflows, and present strategies for intelligently selecting the most important data instances to annotate. Finally, we conclude with some thoughts on the future of crowdsourcing in computer vision.

==> frontmatter.tex <==
%% Front matter for for FnT Computer Graphics & Vision
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[1em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{1.5ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

  \fontsize{13}{15}\selectfont\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\begin{minipage}{\textwidth}
\bfseries\sffamily\Large \@journaltitleprefix\\ \@journaltitle
\end{minipage}

\parskip6pt
\footnotesize

\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

{\raggedright
\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{8pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{\footnotesize
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\fontsize{9}{11}\selectfont
\begin{multicols}{3}
\raggedcolumns
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro\par

\fontsize{10}{13}\selectfont
\begin{multicols}{2}
    \raggedright
    \@journaltopics
\end{multicols}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
\@journaltitleprefix\\ \@journaltitle\par}%
Vol.~\@volume, No.~\@issue\ (\@pubyear) 
\@firstpage--\@lastpage\\
{\hangindent=3.5ex
\hangafter=1
\copyright\ \@copyrightyear\ \@copyrightowner\par}%
DOI: \@doi}\hss
\vbox{\hsize=.4\textwidth 
    \raggedleft
    \includegraphics[width=53bp]{now_logo}\\
    \includegraphics[width=81bp]{essence_logo}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Computer Graphics and Vision}

\journalchiefeditor{\textbf{Brian Curless} \\
University of Washington \\
United States}

\journalchiefeditor{\textbf{William T. Freeman}\\
Massachusetts Institute of Technology \\
United States \columnbreak}

\journalchiefeditor{\textbf{Luc Van Gool} \\
KU Leuven, Belgium \\
ETH Zurich, Switzerland \columnbreak}


\journaleditor{Marc Alexa \\ \emph{TU Berlin}}
\journaleditor{Kavita Bala \\ \emph{Cornell University}}
\journaleditor{Ronen Basri \\ \emph{Weizmann Institute}}
\journaleditor{Peter Belhumeur \\ \emph{Columbia University}}
\journaleditor{Andrew Blake \\ \emph{Microsoft Research}}
\journaleditor{Chris Bregler \\ \emph{Facebook/Oculus}}
\journaleditor{Joachim Buhmann \\ \emph{ETH Zurich}}
\journaleditor{Michael Cohen \\ \emph{Microsoft Research}}
\journaleditor{Paul Debevec \\ \emph{USC ICT}}
\journaleditor{Julie Dorsey \\ \emph{Yale University}}
\journaleditor{Fredo Durand \\ \emph{MIT}
\journaleditor{Olivier Faugeras \\ \emph{INRIA}}
\journaleditor{Rob Fergus \\ \emph{New York University}}
\journaleditor{Mike Gleicher \\ \emph{University of Wisconsin}}}
\journaleditor{Richard Hartley \\ \emph{ANU}\columnbreak}
\journaleditor{Aaron Hertzmann \\ \emph{Adobe Research, USA}}
\journaleditor{Hugues Hoppe \\ \emph{Microsoft Research}}
\journaleditor{C. Karen Liu \\ \emph{Georgia Tech}}
\journaleditor{David Lowe \\ \emph{UBC}}
\journaleditor{Jitendra Malik \\ \emph{UC Berkeley}}
\journaleditor{Steve Marschner \\ \emph{Cornell University}}
\journaleditor{Shree Nayar \\ \emph{Columbia University}}
\journaleditor{James O'Brien \\ \emph{UC Berkeley}}
\journaleditor{Tomas Pajdla \\ \emph{Czech TU}}
\journaleditor{Pietro Perona \\ \emph{Caltech}}
\journaleditor{Marc Pollefeys \\ \emph{ETH Zurich}}
\journaleditor{Jean Ponce \\ \emph{Ecole Normale Sup\'erieure}\columnbreak}
\journaleditor{Long Quan \\ \emph{HKUST}}
\journaleditor{Cordelia Schmid \\ \emph{INRIA}}
\journaleditor{Steve Seitz \\ \emph{University of Washington}}
\journaleditor{Amnon Shashua \\ \emph{Hebrew University}}
\journaleditor{Peter Shirley \\ \emph{University of Utah}}
\journaleditor{Noah Snavely \\ \emph{Cornell University}}
\journaleditor{Stefano Soatto \\ \emph{UCLA}}
\journaleditor{Richard Szeliski \\ \emph{Microsoft Research}}
\journaleditor{Joachim Weickert \\ \emph{Saarland University}}
\journaleditor{Song Chun Zhu \\ \emph{UCLA}}
\journaleditor{Andrew Zisserman \\ \emph{University of Oxford}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles in the following topics:}

\journaltopics{
\begin{itemize}\itemsep=0pt
    \item{Rendering}
    \item{Shape}
    \item{Mesh simplification}
    \item{Animation}
    \item{Sensors and sensing}
    \item{Image restoration and enhancement}
    \item{Segmentation and grouping}
    \item{Feature detection and selection}
    \item{Color processing}
    \item{Texture analysis and synthesis}
    \item{Illumination and reflectance modeling}
    \item{Shape representation}
    \item{Tracking}
    \item{Calibration}
    \item{Structure from motion}
    \item{Motion estimation and registration}
    \item{Stereo matching and reconstruction}
    \item{3D reconstruction and image-based modeling}
    \item{Learning and statistical methods}
    \item{Appearance-based matching}
    \item{Object and scene recognition}
    \item{Face detection and recognition}
    \item{Activity and gesture recognition}
    \item{Image and video retrieval}
    \item{Video analysis and event recognition}
    \item{Medical image analysis}
    \item{Robot localization and navigation}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 4 issues. ISSN paper version 1572-2740. %%% (\@paperprice).
  ISSN online version 1572-2759. %%% (\@onlineprice).
  Also available as a combined paper and online
  subscription.%%% (\@combinedprice).
}

\endinput

